Semantic keypoint-based pose estimation from single RGB frames

This paper presents an approach to estimating the continuous 6-DoF pose of an object from a single RGB image. The approach combines semantic keypoints predicted by a convolutional network (convnet) with a deformable shape model. Unlike prior investigators, we are agnostic to whether the object is textured or textureless, as the convnet learns the optimal representation from the available training-image data. Furthermore, the approach can be applied to instance- and class-based pose recovery. Additionally, we accompany our main pipeline with a technique for semi-automatic data generation from unlabeled videos. This procedure allows us to train the learnable components of our method with minimal manual intervention in the labeling process. Empirically, we show that our approach can accurately recover the 6-DoF object pose for both instance- and class-based scenarios even against a cluttered background. We apply our approach both to several, existing, large-scale datasets - including PASCAL3D+, LineMOD-Occluded, YCB-Video, and TUD-Light - and, using our labeling pipeline, to a new dataset with novel object classes that we introduce here. Extensive empirical evaluations show that our approach is able to provide pose estimation results comparable to the state of the art.

==> old_latex/contributions.tex <==

\vspace{5pt}\noindent{\bf Contributions }In the light of previous work, the contributions of our work are as follows:
\begin{itemize}
\item We present an efficient approach that combines highly reliable (semantic) keypoints predicted by a convnet with a deformable shape model to estimate the continuous 6-DoF pose of an object. Unlike previous work, we are agnostic to whether the object is textured or textureless, as the convnet learns the optimal representation from the available image training data.  Furthermore, the same approach can be applied to instance- and class-based pose recovery.  

\item Empirically, we demonstrate that the proposed approach yields accurate 6-DoF pose estimates in scenes with cluttered backgrounds without the requirement of any pose initialization. State-of-the-art performance is shown on the large-scale PASCAL3D+ dataset \cite{xiang2014}.  
\end{itemize}

==> old_latex/evaluation.tex <==
\subsection{Instance-based pose recovery: gas canister}

This section considers the recovery of pose for a specific object instance. This case fits well with many robotics applications where the objects in the environment are known. Moreover, it allows us to establish the accuracy of our approach in a relatively simple setting before dealing with the more challenging object class scenario.

We collected a dataset of 175 RGB-D images of a textureless gas canister. 
The depth data was only used to generate the groundtruth. More specifically, a complete 3D model of the gas canister was reconstructed using KinectFusion \cite{newcombe2011} and the groundtruth object pose for each image was calculated by ICP with careful manual initialization. Then, 10 keypoints were manually defined on the 3D model and projected to the images yielding groundtruth keypoint locations in 2D for training the convnet. 

A random 85\%/15\% split was used for the training/test data. A stacked hourglass network with two hourglass modules was trained. The output heatmaps for the testing images are visualized in the second column of Fig. \ref{fig:gascan}.  As can be seen, the hourglass network is able to locate the keypoints reliably in the presence of viewpoint variety and occlusions. The non-visible keypoints are also well localized due to the network's ability to take global context into account. The estimated object poses are shown in the last two columns of Fig. \ref{fig:gascan}. The projected 3D models align accurately with the image; the full-perspective solution is more precise than the weak-perspective one. It is worth noting that only 150 images were used to train the network from scratch. Overfitting might be an issue with such a small training set, but the empirical results suggest that the hourglass model captures the object appearance very well in this single instance case. More challenging examples with large intra-class variability are considered in Section \ref{sec:pascal}. 

The 6-DoF pose was estimated with the known 3D model and camera intrinsic parameters using the optimization in Section \ref{sec:optimization}. The following geodesic distance was used to measure the rotation error between a pose estimate, $R_1$, and the groundtruth, $R_2$: 
\begin{align}
\Delta(R_1,R_2) = \frac{\|\log(R_1^TR_2)\|_{F}}{\sqrt{2}}.\label{eq:geodesic}
\end{align}
As a simple baseline, the following greedy approach was implemented: the maximum response locations in the heatmaps were selected as 2D keypoint locations and the standard PnP problem was solved by the EPnP algorithm~\cite{lepetit2009} to estimate the object pose. The results are presented in Table~\ref{tab:gas}. While the weak-perspective solutions (Proposed WP) are on average worse than EPnP due to the inaccurate camera model, the full-perspective solutions (Proposed FP) are much more precise than those of EPnP.  The remarkably small pose errors returned by the proposed approach based on a single RGB image are in the range suitable for a general grasping system. In the supplemental video\footnote{https://www.seas.upenn.edu/\%7Epavlakos/projects/object3d}, we demonstrate the efficacy of our approach in this situation by way of a robot grasping experiment. 

\begin{table}
\caption{Pose estimation errors on the gas canister dataset.}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c*{15}{c}}
\hline
 \multirow{2}{*}{Approach}& \multicolumn{2}{c}{Rotation (degree)} & \multicolumn{2}{c}{Translation (mm)} \\
& Mean & Median & Mean & Median \\
\hline
Proposed WP & 7.99 & 7.61 & N/A & N{}/A \\
Proposed FP & 3.57 & 3.11 & 12.05 & 8.82 \\
EPnP \cite{lepetit2009} & 7.17 & 5.21 & 43.45 & 21.51 \\
\hline
\end{tabular}
\vspace{0.25em}
\label{tab:gas}
\end{table}{}

\begin{figure*}{}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/gascan/valid_16.pdf}\\
  \includegraphics[width=0.8\linewidth]{figures/gascan/valid_12.pdf}\\
  \includegraphics[width=0.8\linewidth]{figures/gascan/valid_24.pdf}\\
  \caption{Qualitative results on the gas canister dataset. From left-to-right: RGB images with bounding boxes provided by Faster R-CNN~\cite{ren2015faster}, heatmaps from the convnet, projections of the 3D model with estimated poses using the weak-perspective model and full-perspective model, respectively. Note the better alignment near the handle with the full-perspective model.}\label{fig:gascan}
\end{figure*}

\subsection{Class-based pose recovery: PASCAL3D+}\label{sec:pascal}

Moving to a more challenging scenario, we demonstrate the full strength of our approach using the large-scale PASCAL3D+ dataset \cite{xiang2014}. The stacked hourglass network was trained from scratch with the training set of PASCAL3D+. Instead of training separate models for different object classes, a single network was trained to output heatmap predictions for all of the 124 keypoints from all classes. Using a single network for all keypoints allows us to share features across the available classes and significantly decreases the number of parameters needed for the network. At test time, given the class of the test object, the heatmaps corresponding to the keypoints belonging to this class were extracted. For pose optimization, two cases were tested: (i) the CAD model for the test image was known; and (ii) the CAD model was unknown and the pose was estimated with a deformable model whose basis was learned by PCA on all CAD models for each class in the dataset. Two principal components were used ($k=2$) for each class, which was sufficient to explain greater than $95\%$ of the shape variation. The 3D model was fit to the 2D keypoints with a weak-perspective model as the camera intrinsic parameters were not available. 

\vspace{5pt}\noindent{\bf Semantic correspondences } A crucial component of our approach is the powerful learning procedure that is particularly successful at establishing correspondences across the semantically related keypoints of each class. To demonstrate this network property,  in Fig.~\ref{fig:semantic} we present a subset of the keypoints for each class along with the localizations of these keypoints in a randomly selected set of images among the ones with the top 50 responses. It is interesting to note that despite the large appearance differences due to extreme viewpoint and intra-class variability, the predictions are very consistent and preserve the semantic relation across various class instances.

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/pascal3d/valid_semKeyp_9.pdf}\\
  \includegraphics[width=\linewidth]{figures/pascal3d/valid_semKeyp_42.pdf}\\
  \includegraphics[width=\linewidth]{figures/pascal3d/valid_semKeyp_50.pdf}\\
  \includegraphics[width=\linewidth]{figures/pascal3d/valid_semKeyp_61.pdf}\\
  \caption{Localization results for diverse keypoint categories. We visualize eight images selected randomly from the top 50 responses for each keypoint. The keypoint localization network is particularly successful at establishing semantic correspondences across the instances of a class, despite the significant intra-class variation and wide ranging camera viewpoints.}\label{fig:semantic}
\end{figure*}

\vspace{5pt}\noindent{\bf Pose estimation } The quantitative evaluation for pose estimation on PASCAL3D+ is presented in Table~\ref{tab:pascal3d}. Only the errors for rotations are reported as the 3D translation cannot be determined in the weak perspective case and the ground truth is not available as well. The rotational error is calculated using the geodesic distance, (\ref{eq:geodesic}). The proposed method shows improvement across most categories with respect to the state-of-the-art. The best results are achieved in the case where the fine subclass for the object is known and there exists an accurate CAD model correspondence. The proposed method with uniform weights for all keypoints is also compared as a baseline, which is apparently worse than considering the confidences during model fitting. A subset of results of the proposed method are visualized in Fig.~\ref{fig:models3d}.

\begin{figure*}
  \centering
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/aeroplane_valid_1243_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/aeroplane_valid_1299_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/bicycle_valid_2475_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/bottle_valid_5534_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/bus_valid_6295_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/car_valid_9982_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/car_valid_10093_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/chair_valid_11274_model.pdf}
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/chair_valid_11447_model.pdf} 
  \includegraphics[width=0.49\linewidth]{figures/pascal3d/sofa_valid_15763_model.pdf} 
   \includegraphics[width=0.49\linewidth]{figures/pascal3d/train_valid_16909_model.pdf}
   \includegraphics[width=0.49\linewidth]{figures/pascal3d/train_valid_16710_model.pdf}
  \caption{Example results of our approach on PASCAL3D+. For each example from left-to-right: 
the RGB image of the object, heatmap responses for the keypoints of the specific class, the CAD model projected to 2D after pose estimation, and the CAD model visualized in 3D.
}\label{fig:models3d}
\end{figure*}

\begin{table*}[t]
\caption{Viewpoint Estimation Median Error (degrees) on PASCAL3D+.}
\begin{center}

\begin{tabular}{c|cccccccccc}
\hline
   Approach    &     aero &       bike &  	 bottle &           bus &           car &         chair &	sofa &         train &         TV monitor  &	boat        \\
\hline
Tulsiani and Malik~\cite{tulsiani2015vk}	&         13.8 &         17.7 &     	12.9 &          5.8 &          9.1 &         14.8 &         15.2 &          8.7 &         {\bf 15.4} &    	{\bf 21.3}  \\
ours - PCA basis  &	11.2 &         15.2 &          13.1 &          4.7 &          6.9 &         12.7 &        21.7 &          9.1 &        38.5 &         37.9   \\
ours - CAD basis 	&   {\bf 8.0} &         {\bf 13.4} &        {\bf 11.7} &          {\bf 2.0} &          {\bf 5.5} &         {\bf 10.4} &          {\bf 9.6} &          {\bf 8.3} &          32.9 &         40.7 \\
ours - uniform weights 	&	16.3 &         17.8 &          14.1 &          11.7 &          30.7 &         17.6 &        32.4 &          20.8 &        25.0 &         72.0   \\
\hline
\end{tabular}

\end{center}
\label{tab:pascal3d}
\end{table*}

\vspace{5pt}\noindent{\bf Failure cases } In Table~\ref{tab:pascal3d} we observed higher errors than the state-of-the-art for two classes, namely boat and TV monitor. For most images of TV monitor, there are only four coplanar keypoints. This makes pose estimation an ill-posed problem for the weak perspective case. Figure \ref{fig:failure} illustrates some failure cases because of this ambiguity. For boat we observed that in many cases the objects are very small and there are insufficient cues to discriminate between the front and the back, which makes the keypoint localization extremely hard. In these extreme cases, holistic and discrete viewpoint prediction might be more robust, which could in practice provide a prior to regularize our continuous prediction. We exclude the results for two classes from PASCAL3D+, namely dining table and motorbike, as we observed some inconsistency of the left-right definition in groundtruth annotations, which lead to erroneous training data. Since other approaches (e.g., \cite{tulsiani2015vk}) rely on discrete viewpoint annotations only, this issue is not reported.

\begin{figure}
  \centering
   \includegraphics[width=\linewidth]{figures/pascal3d/tvmonitor_valid_17604_model.pdf}
   \includegraphics[width=\linewidth]{figures/pascal3d/tvmonitor_valid_17633_model.pdf}\\  
  \caption{Failure cases for the TV monitor class of PASCAL3D+. Although the visible keypoints are localized successfully the pose optimization fails because the 4 points are coplanar and the problem becomes ill-posed.}\label{fig:failure}
\vspace{-1em}
\end{figure}

\subsection{Processing time}
\textcolor{red}{UPDATE}
On a desktop with an Intel i7 3.4GHz CPU, 8G RAM and a GeForce GTX Titan X 6GB GPU, our pipeline needs around 0.2 seconds for the keypoint localization step and less than 0.1 seconds for the shape fitting step, for a total running time under 0.3 seconds. This makes our approach particularly suitable for applications where near real-time is desired. Moreover, further improvements in the running time are anticipated due to improvements in hardware, particularly with GPUs.

==> old_latex/summary.tex <==
In this paper, we proposed an efficient method to estimate the continuous 6-DoF pose of an object from a single RGB image. Capitalizing on the robust semantic keypoint predictions provided by a state-of-the-art convnet, we proposed a pose optimization scheme that fits a deformable shape model to the 2D keypoints and recovers the 6-DoF pose of the object. To ameliorate the effect of false detections, our pose optimization integrates the heatmap response values in the optimization scheme to model the certainty of each detection. Both the weak perspective and the full perspective cases were investigated. The experimental validation included an instance-based scenario as well as full-scale evaluation on the PASCAL3D+ dataset, where we demonstrated state-of-the-art results for viewpoint estimation. Additionally, our method is accompanied by an efficient implementation with a running time under 0.3 seconds, making it a good fit for near real-time robotics applications.

\vspace{1em}

{\bf Acknowledgements:} We gratefully appreciate support through the following grants: NSF-DGE-0966142 (IGERT), NSF-IIP-1439681 (I/UCRC), NSF-IIS-1426840, ARL MAST-CTA W911NF-08-2-0004, ARL RCTA W911NF-10-2-0016, ONR N00014-17-1-2093, an ONR STTR (Robotics Research), NSERC Discovery, and the DARPA FLA program.

==> response.tex <==
\setcounter{section}{0}
\newpage

We thank all the reviewers for their constructive and insightful comments.  Our proposed revisions have been \secondchanges{highlighted} in the revised manuscript.

\section{Response to Reviewer 1's Suggestions}
We add numerous phrasing improvements and standardized notation throughout the paper.

We provide more details about our network architecture and training procedure.  Additionally, we provide a link to our source code.

We incorporate the suggestions to improve the notation in the description of keypoint refinement methods.

We provide additional discussion of our occlusion detection method, and include threshold values related to keypoint refinement.

We provide the number of keypoints for each class in our dataset and add a link to the dataset's website.

We explicitly state which keypoint refinement method performs better and highlight the refinement method comparison as a primary question regarding the semi-automatic annotation pipeline. We re-arrange the paragraph discussing Table 7 and Table 8 in the text to further highlight this comparison. 

We added additional discussion of the experimental setup and the results for the PASCAL3D+ dataset.

We corrected the citations for all of the papers that we cited as being published in arXiv that had been subsequently published in a different venue.

\section{Response to Reviewer 2's Suggestions}
We rephrase the description of our object-level 6DoF experiments, and point out that CosyPose~\cite{labbe2020cosypose} is currently the state-of-the-art method in the BOP benchmark. But we maintain that the performance of our method is competitive with respect to other entries in the benchmark and other methods that are less than a year old. 

We present this manuscript as an extended version of the original conference publication. The main technical novelty remains in using predicted keypoints and basis functions to estimate object pose. We bring the paper up to date by contributing new experiments that show the method's performance in object-level pose estimation. In addition, we address the practical issues of adapting for new objects by proposing a new data generation pipeline that complement the main method. 



